Evaporating Black Holes Coupled to a Thermal Bath

We study the doubly holographic model of [arXiv:1908.10996] in the situation where a black hole in two-dimensional JT gravity theory is coupled to an auxiliary bath system at arbitrary finite temperature. Depending on the initial temperature of the black hole relative to the bath temperature, the black hole can lose mass by emitting Hawking radiation, stay in equilibrium with the bath or gain mass by absorbing thermal radiation from the bath. In all of these scenarios, a unitary Page curve is obtained by applying the usual prescription for holographic entanglement entropy and identifying the quantum extremal surface for the generalized entropy, using both analytical and numeric calculations. As the application of the entanglement wedge reconstruction, we further investigate the reconstruction of the black hole interior from a subsystem containing the Hawking radiation. We examine the roles of the Hawking radiation and also the purification of the thermal bath in this reconstruction.

==> sections/extra.tex <==
% !TEX root = ../FTB_v07.tex

\newpage
\section{Proposed Focus Topics}

\begin{enumerate}
	\item {\bf Introduction:} Short introduction; ends with "The remainder of this paper is organized as follows:".
	%
	\item {\bf Background and setup:}
	%
	\item {\bf Thermal equilibrium ($T_1=\Tb$):}
	\begin{enumerate}
		\item Need to keep (portion of) purification to get a quantum extremal island (QEI).
		\item Page curve is reminiscent of that for state  where bath is prepared in equilibrium with BH in Hartle-Hawking state -- see \cite{Almheiri:2019yqk}.
		\item Keeping the entire purification, we look at `early' and `late' time protocols of  \cite{Chen:2019uhq} and find uberology$^2$?: After the Page time (when the QEI first appears), only need radiation of a segment of length $\Delta\sigma\simeq \frac12\,u_\mt{Page}$ that can be placed anywhere between $\sigma=0$ and $\sigma=\sigma_\mt{shock}\ (=u)$. Further note that $u_\mt{Page}$ is shorter than in the case with $\Tb=0$. Try to explain these puzzles.
		\item Examine of purification is really needed to produce a QE Island. (May help with previous puzzles.)
		\end {enumerate}
		%
		\item {\bf Out of equilibrium ($T_1\ne\Tb$):}
		\begin{enumerate}
			\item BH will reach an equilibrium configuration with $T_\mt{Hawk}=\Tb$. Probably best to examine some examples numerically. Consider both $T_1>\Tb$ and $T_1<\Tb$.
			\smr{solutions of QES at Section 4.2.1, numerical plots at 4.2.2}
			\item Examine Page curve. Should saturate with an entropy $\sim S_\mt{BH}(\Tb)$. What does approach to equilibrium look like? For $T_1\ll \Tb$, should see turnover/behaviour reminiscent of Page curve for $\Tb=0$. (Are there extra phase transitions of the HRT surface in the late time regime??)
			\smr{Page transition at section-4.2.2; diagram for full Page curve locates at section-4.2.5}
			
			\item At $\Tb=0$, there is no purification. So it is interesting to understand how the portion of the purification needed vanishes as $\Tb\to0$, \eg, does the size shrink continuously as $\Tb$ shrinks or is it a `phase transition' where the size goes to zero at a critical bath temperature?
			\smr{The critical temperature requiring purification is shown in section-4.3.2.}
		\end{enumerate}
		%
		\item \rcm{What else is interesting? There are probably an infinite number of possible topics but we should focus to produce a finite-size and finite-time project.}
		%
		\item {\bf Discussion:} We discuss stuff. For now, we should simply collect a list of discussion worthy topics/ideas. 
	\end{enumerate}
	
	\section{Interesting discussion points:}
	\rcm{What did we learn here?}
	
	\begin{itemize}
		%
		\item \textbf{Doubly holographic model:} Just like the previously studied evaporating models of~\cite{Almheiri:2019hni,Chen:2019uhq}the system studied in this paper has three descriptions in models in different dimensions. In the ground level, it can be thought of as the TFD in a holographic QM dual to JT gravity plus a holograhpic CFT in $AdS_2$. One of the two halfs of the TFD is then put into contact with CFT matter in a bath with a finite temperature $T_b$ and the system equilibrates with time. On the first holographic level, we have a black hole in JT gravity plus CFT matter in equilibrium with the black hole geometry. The double sided black hole geometry is then coupled to a finite temperature bath through one of its asymptotic boundaries. The second (doubly) holographic level consist of a planck brane in which the JT gravity is located and Einstein gravity in a bulk $AdS_3$ dual to the CFT matter in both the plank brane and the bath. The bath is initially separated by an end-of-the-world brane which pinches off as the two systems are coupled together.
		
		\item \textbf{Three phases of evaporation:} Just like in the zero temperature bath model studied in~\cite{Chen:2019uhq}, we find three phases in the process of a black thermalizing with a finite temperature bath: the quench phase, the scrambling phase and the late-time phase.
		
		\item \textbf{Quench phase:} Similar to the zero temperature case, the von Neumann entropy in the scrambling case is independent of the position of the extremal surface, which immediately implies that the quantum extremal surface remains at the bifurcation point for this phase. From the first holographic level, the increase in entropy is due to the exchange of Hawking modes between bath and black hole, which is why the linear increase is proportional to $T_1+T_b$. From the doubly holographic perspective, the increase in generalized entropy is purely related to the end-of-the-world brane falling off deeper into the bulk, the speed of this falloff is controlled by the temperature of the black hole and of the bath. 
		
		\item \textbf{Late-time phase:} After the Page time, we encounter the late-time phase in which equilibration occurs. For a bath with a temperature which matches that of the post-quench black hole $T_b=T_1$, this equilibration is immediate and the generalized entropy is constant in this phase. The von Neummann entropy of the matter fields is identical to those of a CFT in the eternally coupled case of~\cite{Almheiri:2019yqk}, and the geometry is also identical. This is to be expected at since the system has equilibrated with the bath and therefore the time when the coupling of the two was done is irrelevant from the point of view of the entanglement entropy \jh{Would more fine grained measures of entanglement potentially be sensible to this? Renyi entropies, complexity?}.
		
		\item \textbf{Position of the QES:} The position of the late-time extremal surface relative to the event horizon of the black hole depends on the temperature of the bath. In the evaporating models ($T_b=0$) of~\cite{Almheiri:2019psf,Almheiri:2019hni,Chen:2019uhq}, the late-time extremal surface is \emph{behind} the horizon. Correspondingly, the information of the geometry outside of the black hole could not be reconstructed by \QML + bath. On the other hand, in the eternally coupled case of~\cite{Almheiri:2019yqk}, the extremal surface is instead located \emph{outside} of the event horizon. Similarly, in the equilibrium case studied in section~\ref{sec:equilibrium}, the late-time extremal surface is located outside the event horizon. The information just outside of the event horizon could therefore be reconstructed by \QML + bath after the Page time. Moreover, for \emph{any} temperature, the black hole eventually equilibrates with the bath, and the system is qualitatively similar to the equilibrium case. Indeed, for any temperature, after a time of $ku \geq \log\left(\left|1-\frac{T_1^2}{T_b^2}\right| \sqrt{\frac{\pi T_1}{8k}}\right)$, the late-time extremal surface crosses the horizon and stays outside as the system equilibrates. Furthermore, for bath temperatures very close to $T_1$, \ie $\frac{|T_b-T_1|}{T_1} \leq  \sqrt{\frac{2k}{\pi T_1}} e^{\frac{T_1-T_0}{2T_1}}$, the late time extremal surface is already outside of the event horizon by the Page time.
		
		\item \textbf{Importance of the purification:} Studying the entanglement structure of the equilibrium setup of section~\ref{sec:equilibrium}, we found that the reconstruction of black hole interior \emph{always} required at least part of the purification of the bath. This is in contrast from the results of the evaporation black hole to a zero temperature bath, where, trivially, the purification is not needed. We found that the temperature at which the purification becomes essential for interior reconstruction is $T_b= T_p$ which is very close to $T_1$. This need for the purification of the bath is due to the infalling radiation from the bath to the black hole having enough of an effect on the black hole interior by the Page time that their respective entangled modes in the purification are needed to reconstruct the interior. The fact that $T_p$ is close to $T_1$ reflect the fact that the bath has to have around the same mount of radiation falling into the black hole as the black hole was emitting. This is to be expected because, when the two are radiating away at roughly the same rate, one would expect that when the black hole has radiated away enough information to allow it's interior be reconstructed, a bath emitting the same amount of radiation into the black hole could have entangled the said black hole with its purification.
		
		\item {\bf Spread of Information via entanglement}
		
		\item \textbf{Effective temperature:} The effective temperature  in eq.~\eqref{eq:Teff} appears everywhere in our calculations, and indeed the late-time generalize entropy in eq.~\eqref{Sgen_late_analytical} has a remarkably simple expression in terms of the effective temperature. Essentially, this effective temperature keeps track of the current temperature of the black hole during the equilibration process.
		
		\item \textbf{Stretched horizon:}
		
		\item Many of the expressions in our analysis take a simple form when expressed in terms of the effective temperature in eq.~\eqref{eq:Teff}, ranging from the energy and the Schwarzian in eqs.~\eqref{eq:energy} and \eqref{eq:chocolate}, and even the late-time generalize entropy in eq.~\eqref{Sgen_late_analytical} has a remarkably simple expression in terms of the effective temperature. This effective temperature keeps track of the current temperature of the black hole during the equilibration process. \jh{Strictly speaking the system isn't in equilibrium. Should we consider this ``momentary temperature'' as the temperature the resulting black hole would have if we performed a splitting quench at the given time? Or is there another sense in which the $T_{\rm eff}$ can indeed be considered the temperature of the AdS subsystem?}\smr{The effective temperature is directly related to the ADM mass for the AdS system (see \eqref{eq:energy}). We can understand the temperature $T_{\rm{eff}}(u)$ from the viewpoint of the energy of system. On the other hand, if we consider the stress tensor, the effective temperature $T_{\rm{eff}}(u)$ can be understood as the temperature of the Hawking radiation at time $u$ (see eq (3.24)).}.
		%
		
		\item Page time \\
		\jh{Do we agree with this explanation?:} As was noted around eq.~\eqref{eq:pagetime}, the dependence of the Page time on the bath temperature is not monotonic. The Page time decreases as $T_b$ starts from zero and grows to the equilibrium case $T_b=T_1$, after which the Page time decreases as the $T_b$ keeps increasing. We attribute this behavior to two competing effects. Firstly, the flux of information between the bath and the black hole system increases with $T_b$ simply because the bath radiation falling into the black hole increases with $T_b$. This increase in information flux causes the Page transition at an earlier time, as can be seen in the increasing slope of the scrambling phase generalized entropy in figure~\ref{fig:Sgen3T1_pagetime}. The second and competing effect is that with higher $T_b$, the infalling thermal radiation from the bath causes the black hole interior to contain more information. The {\QML}+bath system would correspondingly require more time to have enough information to recover the interior of the black hole as $T_b$ increases. This effect can be visualized by the increasing entropy at the page time as a function of $T_b$ in figure~\ref{fig:Sgen3T1_pagetime}. It is through these two competing effects that the Page time exhibits the aforementioned behaviour with with the bath temperature.
	\end{itemize}
	
	\textcolor{red}{Missing:}
	
	\begin{itemize}
		\item Stretched horizon discussion
		\item Vincent had some interesting things about how much of the purification is needed in the equilibrium case in section~\ref{sec:equilibrium}
	\end{itemize}
